3DCoMPaT200: Language-Grounded Compositional Understanding of Parts and Materials of 3D Shapes

Understanding objects in 3D at the part level is essential for humans and robots to navigate and interact with the environment. Current datasets for part-level 3D object understanding encompass a limited range of categories. For instance, the ShapeNet-Part and PartNet datasets only include 16, and 24 object categories respectively. The 3DCoMPaT dataset, specifically designed for compositional understanding of parts and materials, contains only 42 object categories. To foster richer and fine-grained part-level 3D understanding, we introduce 3DCoMPaT200, a large-scale dataset tailored for compositional understanding of object parts and materials, with 200 object categories with $\approx$5 times larger object vocabulary compared to 3DCoMPaT and $\approx$ 4 times larger part categories. Concretely, 3DCoMPaT200 significantly expands upon 3DCoMPaT, featuring 1,031 fine-grained part categories and 293 distinct material classes for compositional application to 3D object parts. Additionally, to address the complexities of compositional 3D modeling, we propose a novel task of Compositional Part Shape Retrieval using ULIP to provide a strong 3D foundational model for 3D Compositional Understanding. This method evaluates the model shape retrieval performance given one, three, or six parts described in text format. These results show that the model's performance improves with an increasing number of style compositions, highlighting the critical role of the compositional dataset. Such results underscore the dataset's effectiveness in enhancing models' capability to understand complex 3D shapes from a compositional perspective. Code and Data can be found at http://github.com/3DCoMPaT200/3DCoMPaT200

==> sec/method.tex <==
\section{Method}
To facilitate 3D part and material understanding, we build a 3D segmentation network based on vision-language alignment and a Hubless loss to address class imbalance. As illustrated in Fig.~\ref{fig_overview}, our method consists of four key components, a 3D encoder, a text encoder, contrastive vision-language loss, and Vilhub loss.

\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth,height=6cm]{figs/fig_overview.pdf}
    \caption{Method Overview. Our part/material segmentation network consists of a 3D encoder, and a text encoder, and is trained using a vision-language contrastive loss and Vilhub loss.}
    \label{fig_overview}
\end{figure}

\noindent \textbf{3D Encoder.}
Given a three-dimensional point set $P \in \mathbb{R}^{N \times 6}$, consisting of $N$ points, where each point is characterized by its three-dimensional coordinates and associated colors, we employ an encoder network $E_P$ to extract point features, denoted as $\{f^V_i\}_{i=1}^N = E_P (P)$. In our experiments, various visual backbones are explored to extract point features from raw point clouds effectively. Furthermore, to separate geometric from appearance features, we have designed two distinct heads within our framework, specifically dedicated to the segmentation of parts and materials. This dual-head design facilitates the independent analysis of geometric and appearance-based features.
 
\noindent \textbf{Text Encoder.}
In our work, we utilize a pre-trained CLIP~\cite{clip} model to associate parts (materials) with their corresponding text embeddings. It should be noted that the proposed method does not depend on a specific language encoder; however, the multi-modal training capabilities of CLIP can be beneficial for our language-to-3D alignment.

Throughout the training phase, we employ names of parts (materials) as language prompts and apply the pre-trained CLIP model to translate them into text embeddings, denoted by $f^T \in \mathbb{R}^D$, where $D$ denotes the dimensionality of the embedding space. This strategy allows us to harness text features to guide the learning process for 3D features, ensuring that the acquired 3D features are closely aligned with their text encodings in the semantic space when they correspond to the same part (material) category.

\noindent \textbf{Contrastive Vision-Language Supervision.}
Traditional methods of 3D visual understanding predominantly utilize vanilla one-hot labels for training supervision. In this work, to address the long-tail challenge inherent in the 3DCoMPaT200 dataset, we leverage vision-language supervision to align point features with text descriptions in the embedding space. To achieve this, we adopt the approach of CLIP~\cite{clip}, utilizing a contrastive vision-language loss defined below,
\begin{equation}
    p_{ic} = \frac{\exp(<f_i^V, f^T_c>/\tau)}{\sum_{j=1}^C \exp(<f_i^V, f^T_j>/\tau)}, \quad s.t., c \in [1,2,...C]
\end{equation}
\begin{equation}
    \mathcal{L}_{vl} = \text{CE}(p_i, y_i),
\end{equation}
where $f^V_i$ and $f^T$ are pre-normalized, <,> denotes dot product, $\tau$ is a scaling hyperparamter, $p_{ic}$ denotes predicted classification probability for point $p_i$ over class $c$, CE denotes cross-entropy loss, $y_i$ is the ground truth part (material) label for $i$-th point.

\noindent \textbf{Vilhub Loss}
To further address the class imbalance issue, we take inspiration from~\cite{abdelkarim2021exploring} to design a vision-language hubless loss (VilHub). The VilHub tackles the long-tail issue by refining the representations in both language and vision domains through an integrated end-to-end approach. The foundational concept behind our VilHub loss is to promote balanced predictions across both head and tail classes. Given point label prediction $\{p_{ic}\}_{i=1}^N$, the VilHub is calculated as,
\begin{equation}
    p_c = \frac{1}{N} \sum_{i=1}^N p_{ic}, \quad
    \mathcal{L}_{h} = \sum_{c=1}^C (p_c - 1/C)^2
\end{equation}
where $C$ denotes the total number of part (material) classes. $p_c$ is the class preference calculated based on the average likelihood of that category being predicted within the current mini-batch. Based on the definition, VilHub loss naturally encourages an equal preference for all categories, including both dominant and underrepresented ones. 

The final training objective is defined as,
\begin{equation}
    \mathcal{L} = \mathcal{L}_{vl} + \gamma \mathcal{L}_h,
\end{equation}

where $\gamma$ is a scaling factor. The first term $\mathcal{L}_{vl}$ encourages each point to be correctly classified in the embedding space, while the second term $\mathcal{L}_h$ encourages a uniform prediction over both head and tail classes.


